How to Schedule Near-Optimally under Real-World Constraints

Scheduling is a critical part of practical computer systems, and scheduling has also been extensively studied from a theoretical perspective. Unfortunately, there is a gap between theory and practice, as the optimal scheduling policies presented by theory can be difficult or impossible to perfectly implement in practice. In this work, we use recent breakthroughs in queueing theory to begin to bridge this gap. We show how to translate theoretically optimal policies -- which provably minimize mean response time (a.k.a. latency) -- into near-optimal policies that are easily implemented in practical settings. Specifically, we handle the following real-world constraints: - We show how to schedule in systems where job sizes (a.k.a. running time) are unknown, or only partially known. We do so using simple policies that achieve performance very close to the much more complicated theoretically optimal policies. - We show how to schedule in systems that have only a limited number of priority levels available. We show how to adapt theoretically optimal policies to this constrained setting and determine how many levels we need for near-optimal performance. - We show how to schedule in systems where job preemption can only happen at specific checkpoints. Adding checkpoints allows for smarter scheduling, but each checkpoint incurs time overhead. We give a rule of thumb that near-optimally balances this tradeoff.

==> tikz/hills_data.tex <==
\newcommand{\serptNoInfo}{(0.0,0.21148002856278514)--(3.90625e-3,0.21098936557645379)--(7.8125e-3,0.2111885692094655)--(1.171875e-2,0.21215748274676763)--(1.5625e-2,0.213974172207699)--(1.953125e-2,0.216712429068194)--(2.34375e-2,0.2204384581285104)--(2.734375e-2,0.2252064431508353)--(3.125e-2,0.231052708032681)--(3.515625e-2,0.23798832006548973)--(3.90625e-2,0.24599026052117365)--(4.296875e-2,0.2549917530640915)--(4.6875e-2,0.2648729877524368)--(5.078125e-2,0.2754542148490949)--(5.46875e-2,0.2864937823190689)--(5.859375e-2,0.29769379430392495)--(6.25e-2,0.3087152834722929)--(6.640625e-2,0.31920292236883596)--(7.03125e-2,0.3288166239703761)--(7.421875e-2,0.3372647622615331)--(7.8125e-2,0.34433236226182606)--(8.203125e-2,0.349898335269034)--(8.59375e-2,0.3539386098926916)--(8.984375e-2,0.356515754078031)--(9.375e-2,0.3577588848116192)--(9.765625e-2,0.35783921945321306)--(0.1015625,0.3569463398405728)--(0.10546875,0.355268705121528)--(0.109375,0.3529800314256969)--(0.11328125,0.3502315424481985)--(0.1171875,0.3471490949034372)--(0.12109375,0.3438337855417629)--(0.125,0.3403646765640321)--(0.12890625,0.33680253138775657)--(0.1328125,0.3331937763401069)--(0.13671875,0.3295742031954113)--(0.140625,0.3259721621449484)--(0.14453125,0.3224111575411712)--(0.1484375,0.31891185898834445)--(0.15234375,0.31549359325292947)--(0.15625,0.31217540319108034)--(0.16015625,0.3089767610022316)--(0.1640625,0.3059180139081561)--(0.16796875,0.30302062705461086)--(0.171875,0.300307274774252)--(0.17578125,0.29780181923258986)--(0.1796875,0.2955292055661857)--(0.18359375,0.2935152948396374)--(0.1875,0.29178665005841653)--(0.19140625,0.2903702855371314)--(0.1953125,0.2892933856504823)--(0.19921875,0.28858299503719376)--(0.203125,0.28826567850262486)--(0.20703125,0.2883671451558604)--(0.2109375,0.28891182785277686)--(0.21484375,0.28992240605777675)--(0.21875,0.2914192581566128)--(0.22265625,0.2934198285262439)--(0.2265625,0.2959378958627743)--(0.23046875,0.29898273302772865)--(0.234375,0.302558155673286)--(0.23828125,0.30666146778012865)--(0.2421875,0.3112823274343878)--(0.24609375,0.3164015757350351)--(0.25,0.32199009503643483)--(0.25390625,0.328007788171474)--(0.2578125,0.3344027949585314)--(0.26171875,0.3411110818325885)--(0.265625,0.3480565492704328)--(0.26953125,0.35515179363489147)--(0.2734375,0.3622996296538414)--(0.27734375,0.36939542394137637)--(0.28125,0.37633021013438156)--(0.28515625,0.3829944596393526)--(0.2890625,0.3892822821047641)--(0.29296875,0.39509574451466223)--(0.296875,0.4003489460637751)--(0.30078125,0.4049714824638188)--(0.3046875,0.40891098396558645)--(0.30859375,0.4121345105335615)--(0.3125,0.4146287186707215)--(0.31640625,0.41639885373645513)--(0.3203125,0.41746674468465733)--(0.32421875,0.4178680656198404)--(0.328125,0.41764917037927507)--(0.33203125,0.41686380278082763)--(0.3359375,0.41556994495223065)--(0.33984375,0.4138270027850284)--(0.34375,0.41169345536905605)--(0.34765625,0.40922502633603736)--(0.3515625,0.4064733775322412)--(0.35546875,0.40348528331648625)--(0.359375,0.4003022175050101)--(0.36328125,0.3969602726569732)--(0.3671875,0.39349032990349353)--(0.37109375,0.3899184034749588)--(0.375,0.38626609439923393)--(0.37890625,0.38255110006955095)--(0.3828125,0.3787877387543405)--(0.38671875,0.37498745951877344)--(0.390625,0.3711593178398975)--(0.39453125,0.3673104051895931)--(0.3984375,0.3634462270466898)--(0.40234375,0.3595710283440834)--(0.40625,0.35568806849522777)--(0.41015625,0.3517998501374766)--(0.4140625,0.3479083068304813)--(0.41796875,0.34401495538409277)--(0.421875,0.3401210184562855)--(0.42578125,0.3362275227160024)--(0.4296875,0.3323353773325448)--(0.43359375,0.3284454369252785)--(0.4375,0.32455855245164533)--(0.44140625,0.32067561287276236)--(0.4453125,0.3167975798423356)--(0.44921875,0.312925517131581)--(0.453125,0.3090606160367455)--(0.45703125,0.30520421761708244)--(0.4609375,0.3013578322766839)--(0.46484375,0.29752315692854875)--(0.46875,0.29370208975832424)--(0.47265625,0.28989674243316743)--(0.4765625,0.2861094494736941)--(0.48046875,0.2823427744202545)--(0.484375,0.2785995123757056)--(0.48828125,0.2748826884926897)--(0.4921875,0.27119555199150197)--(0.49609375,0.26754156534200885)--(0.5,0.26392438831632653)--(0.50390625,0.2603478567139348)--(0.5078125,0.2568159556727078)--(0.51171875,0.2533327876023795)--(0.515625,0.24990253490513206)--(0.51953125,0.24652941777499432)--(0.5234375,0.24321764748740204)--(0.52734375,0.23997137569709764)--(0.53125,0.236794640352005)--(0.53515625,0.2336913088997333)--(0.5390625,0.23066501951059104)--(0.54296875,0.22771912106693795)--(0.546875,0.22485661267585344)--(0.55078125,0.222080083454681)--(0.5546875,0.21939165332281088)--(0.55859375,0.2167929155149051)--(0.5625,0.21428488151806588)--(0.56640625,0.2118679291354657)--(0.5703125,0.20954175439821066)--(0.57421875,0.20730532809067093)--(0.578125,0.20515685772492434)--(0.58203125,0.2030937558971364)--(0.5859375,0.2011126160788898)--(0.58984375,0.19920919703187887)--(0.59375,0.197378417172802)--(0.59765625,0.19561436034006488)--(0.6015625,0.19391029450421246)--(0.60546875,0.19225870499558037)--(0.609375,0.19065134376912168)--(0.61328125,0.18907929606124396)--(0.6171875,0.1875330654928323)--(0.62109375,0.18600267821833877)--(0.625,0.18447780610432876)--(0.62890625,0.182947908146956)--(0.6328125,0.18140238842786072)--(0.63671875,0.1798307679021745)--(0.640625,0.17822286627001913)--(0.64453125,0.17656898918059666)--(0.6484375,0.17486011514426203)--(0.65234375,0.1730880758757769)--(0.65625,0.17124572344836164)--(0.66015625,0.16932707767311128)--(0.6640625,0.16732744757355547)--(0.66796875,0.1652435217054213)--(0.671875,0.16307342334004946)--(0.67578125,0.16081672810831205)--(0.6796875,0.15847444347727785)--(0.68359375,0.15604895126796084)--(0.6875,0.15354391617485583)--(0.69140625,0.15096416478073632)--(0.6953125,0.14831554076135228)--(0.69921875,0.1456047427679556)--(0.703125,0.14283915182692886)--(0.70703125,0.14002665501406536)--(0.7109375,0.13717547169306765)--(0.71484375,0.134293987829375)--(0.71875,0.13139060289467186)--(0.72265625,0.1284735927630141)--(0.7265625,0.12555099085987975)--(0.73046875,0.1226304887406091)--(0.734375,0.11971935630608507)--(0.73828125,0.11682438105186901)--(0.7421875,0.11395182511306647)--(0.74609375,0.11110739841410916)--(0.75,0.10829624594976107)--(0.75390625,0.10552294709071358)--(0.7578125,0.10279152479821638)--(0.76171875,0.10010546271928629)--(0.765625,9.746772828972354e-2)--(0.76953125,9.488080017158633e-2)--(0.7734375,9.234669857372432e-2)--(0.77734375,8.986701723149078e-2)--(0.78125,8.744295604207744e-2)--(0.78515625,8.507535355618646e-2)--(0.7890625,8.27647187094966e-2)--(0.79296875,8.051126133585278e-2)--(0.796875,7.831492113769399e-2)--(0.80078125,7.6175394898844e-2)--(0.8046875,7.4092161812327e-2)--(0.80859375,7.2064506863853e-2)--(0.8125,7.009154226280585e-2)--(0.81640625,6.817222694972874e-2)--(0.8203125,6.630538423509827e-2)--(0.82421875,6.44897176409572e-2)--(0.828125,6.272382502685056e-2)--(0.83203125,6.100621108620409e-2)--(0.8359375,5.93352983002654e-2)--(0.83984375,5.770943643515149e-2)--(0.84375,5.6126910664304884e-2)--(0.84765625,5.458594839446406e-2)--(0.8515625,5.308472486862341e-2)--(0.85546875,5.162136761477065e-2)--(0.859375,5.019395980473884e-2)--(0.86328125,4.880054258351719e-2)--(0.8671875,4.743911642596566e-2)--(0.87109375,4.6107641575256146e-2)--(0.875,4.480403761558555e-2)--(0.87890625,4.352618223094106e-2)--(0.8828125,4.2271909202045224e-2)--(0.88671875,4.1039005695225554e-2)--(0.890625,3.982520889996143e-2)--(0.89453125,3.8628202076481655e-2)--(0.8984375,3.744561008113926e-2)--(0.90234375,3.6274994445594434e-2)--(0.90625,3.5113848096275053e-2)--(0.91015625,3.3959589813286076e-2)--(0.9140625,3.2809558543087175e-2)--(0.91796875,3.166100769688199e-2)--(0.921875,3.0511099586834615e-2)--(0.92578125,2.935690017471202e-2)--(0.9296875,2.8195374332281965e-2)--(0.93359375,2.702338183912779e-2)--(0.9375,2.5837674370953752e-2)--(0.94140625,2.4634893758889206e-2)--(0.9453125,2.3411571826550747e-2)--(0.94921875,2.2164132134922795e-2)--(0.953125,2.0888893983663656e-2)--(0.95703125,1.958207902838213e-2)--(0.9609375,1.823982087458487e-2)--(0.96484375,1.6858177996562345e-2)--(0.96875,1.5433150300838564e-2)--(0.97265625,1.396069960535211e-2)--(0.9765625,1.2436774234372845e-2)--(0.98046875,1.0857337833087627e-2)--(0.984375,9.218402383523575e-3)--(0.98828125,7.516065254672036e-3)--(0.9921875,5.746549947122134e-3)--(0.99609375,3.9062499999629532e-3)}
\newcommand{\gittinsNoInfo}{(0.0,0.1031995525023907)--(3.90625e-3,9.87627707859307e-2)--(7.8125e-3,9.471947751044202e-2)--(1.171875e-2,9.09444178916228e-2)--(1.5625e-2,8.761155916482889e-2)--(1.953125e-2,8.460952859511137e-2)--(2.34375e-2,8.201103562138982e-2)--(2.734375e-2,7.97932130155759e-2)--(3.125e-2,7.794006087196749e-2)--(3.515625e-2,7.648940528221085e-2)--(3.90625e-2,7.5374952003351e-2)--(4.296875e-2,7.46653206702062e-2)--(4.6875e-2,7.427055929582686e-2)--(5.078125e-2,7.487822860356463e-2)--(5.46875e-2,7.697909550128756e-2)--(5.859375e-2,8.078377190693452e-2)--(6.25e-2,8.662609698222175e-2)--(6.640625e-2,9.500329403826895e-2)--(7.03125e-2,0.10663745112553291)--(7.421875e-2,0.12256849602002577)--(7.8125e-2,0.1442945727845081)--(8.203125e-2,0.17398457317772123)--(8.59375e-2,0.21480101696059517)--(8.984375e-2,0.2713910110937891)--(9.375e-2,0.3127342178481573)--(9.765625e-2,0.31197291025955887)--(0.1015625,0.3096689644188236)--(0.10546875,0.30610358365068085)--(0.109375,0.3015489517795052)--(0.11328125,0.2962483341331832)--(0.1171875,0.2904065326025648)--(0.12109375,0.28416106509793565)--(0.125,0.2776193490898706)--(0.12890625,0.2709233895568872)--(0.1328125,0.26414602107038304)--(0.13671875,0.2573413485496276)--(0.140625,0.2505162878157607)--(0.14453125,0.2436786254523703)--(0.1484375,0.2369122254614237)--(0.15234375,0.23023936109927556)--(0.15625,0.2236466278883048)--(0.16015625,0.21711781145786244)--(0.1640625,0.21074144173506765)--(0.16796875,0.20453565980355687)--(0.171875,0.198423619502787)--(0.17578125,0.19250181164978167)--(0.1796875,0.1868046948158245)--(0.18359375,0.1812570808439098)--(0.1875,0.17593897512175777)--(0.19140625,0.1708934501095147)--(0.1953125,0.16601082143897433)--(0.19921875,0.16142360880357323)--(0.203125,0.1570937815656742)--(0.20703125,0.1530028284230158)--(0.2109375,0.14924006361533293)--(0.21484375,0.14567575672166874)--(0.21875,0.1424498613195432)--(0.22265625,0.13946879550698832)--(0.2265625,0.13679277560889627)--(0.23046875,0.1343926320822505)--(0.234375,0.1322719002839749)--(0.23828125,0.13044552712231172)--(0.2421875,0.12887954637102908)--(0.24609375,0.1276165277082271)--(0.25,0.12660014506489123)--(0.25390625,0.1258879376499621)--(0.2578125,0.12541213207288446)--(0.26171875,0.1252885456495732)--(0.265625,0.12610211376084715)--(0.26953125,0.1280280365024483)--(0.2734375,0.13115297821567748)--(0.27734375,0.13559957343246443)--(0.28125,0.14153277309768053)--(0.28515625,0.14916844270346594)--(0.2890625,0.15878481655884585)--(0.29296875,0.17073763228903105)--(0.296875,0.18548006470958145)--(0.30078125,0.20358897815661062)--(0.3046875,0.22579956278054386)--(0.30859375,0.2530511719003572)--(0.3125,0.28654821749619913)--(0.31640625,0.32784142797840155)--(0.3203125,0.37893679660509644)--(0.32421875,0.4178680656198404)--(0.328125,0.41764917037927507)--(0.33203125,0.41686380278082763)--(0.3359375,0.41556994495223065)--(0.33984375,0.4138270027850284)--(0.34375,0.41169345536905605)--(0.34765625,0.40922502633603736)--(0.3515625,0.4064733775322412)--(0.35546875,0.40348528331648625)--(0.359375,0.4003022175050101)--(0.36328125,0.3969602726569732)--(0.3671875,0.39349032990349353)--(0.37109375,0.3899184034749588)--(0.375,0.38626609439923393)--(0.37890625,0.38255110006955095)--(0.3828125,0.3787877387543405)--(0.38671875,0.37498745951877344)--(0.390625,0.3711593178398975)--(0.39453125,0.3673104051895931)--(0.3984375,0.3634462270466898)--(0.40234375,0.3595710283440834)--(0.40625,0.35568806849522777)--(0.41015625,0.3517998501374766)--(0.4140625,0.3479083068304813)--(0.41796875,0.34401495538409277)--(0.421875,0.3401210184562855)--(0.42578125,0.3362275227160024)--(0.4296875,0.3323353773325448)--(0.43359375,0.3284454369252785)--(0.4375,0.32455855245164533)--(0.44140625,0.32067561287276236)--(0.4453125,0.3167975798423356)--(0.44921875,0.312925517131581)--(0.453125,0.3090606160367455)--(0.45703125,0.30520421761708244)--(0.4609375,0.3013578322766839)--(0.46484375,0.29752315692854875)--(0.46875,0.29370208975832424)--(0.47265625,0.28989674243316743)--(0.4765625,0.2861094494736941)--(0.48046875,0.2823427744202545)--(0.484375,0.2785995123757056)--(0.48828125,0.2748826884926897)--(0.4921875,0.27119555199150197)--(0.49609375,0.26754156534200885)--(0.5,0.26392438831632653)--(0.50390625,0.2603478567139348)--(0.5078125,0.2568159556727078)--(0.51171875,0.2533327876023795)--(0.515625,0.24990253490513206)--(0.51953125,0.24652941777499432)--(0.5234375,0.24321764748740204)--(0.52734375,0.23997137569709764)--(0.53125,0.236794640352005)--(0.53515625,0.2336913088997333)--(0.5390625,0.23066501951059104)--(0.54296875,0.22771912106693795)--(0.546875,0.22485661267585344)--(0.55078125,0.222080083454681)--(0.5546875,0.21939165332281088)--(0.55859375,0.2167929155149051)--(0.5625,0.21428488151806588)--(0.56640625,0.2118679291354657)--(0.5703125,0.20954175439821066)--(0.57421875,0.20730532809067093)--(0.578125,0.20515685772492434)--(0.58203125,0.2030937558971364)--(0.5859375,0.2011126160788898)--(0.58984375,0.19920919703187887)--(0.59375,0.197378417172802)--(0.59765625,0.19561436034006488)--(0.6015625,0.19391029450421246)--(0.60546875,0.19225870499558037)--(0.609375,0.19065134376912168)--(0.61328125,0.18907929606124396)--(0.6171875,0.1875330654928323)--(0.62109375,0.18600267821833877)--(0.625,0.18447780610432876)--(0.62890625,0.182947908146956)--(0.6328125,0.18140238842786072)--(0.63671875,0.1798307679021745)--(0.640625,0.17822286627001913)--(0.64453125,0.17656898918059666)--(0.6484375,0.17486011514426203)--(0.65234375,0.1730880758757769)--(0.65625,0.17124572344836164)--(0.66015625,0.16932707767311128)--(0.6640625,0.16732744757355547)--(0.66796875,0.1652435217054213)--(0.671875,0.16307342334004946)--(0.67578125,0.16081672810831205)--(0.6796875,0.15847444347727785)--(0.68359375,0.15604895126796084)--(0.6875,0.15354391617485583)--(0.69140625,0.15096416478073632)--(0.6953125,0.14831554076135228)--(0.69921875,0.1456047427679556)--(0.703125,0.14283915182692886)--(0.70703125,0.14002665501406536)--(0.7109375,0.13717547169306765)--(0.71484375,0.134293987829375)--(0.71875,0.13139060289467186)--(0.72265625,0.1284735927630141)--(0.7265625,0.12555099085987975)--(0.73046875,0.1226304887406091)--(0.734375,0.11971935630608507)--(0.73828125,0.11682438105186901)--(0.7421875,0.11395182511306647)--(0.74609375,0.11110739841410916)--(0.75,0.10829624594976107)--(0.75390625,0.10552294709071358)--(0.7578125,0.10279152479821638)--(0.76171875,0.10010546271928629)--(0.765625,9.746772828972354e-2)--(0.76953125,9.488080017158633e-2)--(0.7734375,9.234669857372432e-2)--(0.77734375,8.986701723149078e-2)--(0.78125,8.744295604207744e-2)--(0.78515625,8.507535355618646e-2)--(0.7890625,8.27647187094966e-2)--(0.79296875,8.051126133585278e-2)--(0.796875,7.831492113769399e-2)--(0.80078125,7.6175394898844e-2)--(0.8046875,7.4092161812327e-2)--(0.80859375,7.2064506863853e-2)--(0.8125,7.009154226280585e-2)--(0.81640625,6.817222694972874e-2)--(0.8203125,6.630538423509827e-2)--(0.82421875,6.44897176409572e-2)--(0.828125,6.272382502685056e-2)--(0.83203125,6.100621108620409e-2)--(0.8359375,5.93352983002654e-2)--(0.83984375,5.770943643515149e-2)--(0.84375,5.6126910664304884e-2)--(0.84765625,5.458594839446406e-2)--(0.8515625,5.308472486862341e-2)--(0.85546875,5.162136761477065e-2)--(0.859375,5.019395980473884e-2)--(0.86328125,4.880054258351719e-2)--(0.8671875,4.743911642596566e-2)--(0.87109375,4.6107641575256146e-2)--(0.875,4.480403761558555e-2)--(0.87890625,4.352618223094106e-2)--(0.8828125,4.2271909202045224e-2)--(0.88671875,4.1039005695225554e-2)--(0.890625,3.982520889996143e-2)--(0.89453125,3.8628202076481655e-2)--(0.8984375,3.744561008113926e-2)--(0.90234375,3.6274994445594434e-2)--(0.90625,3.5113848096275053e-2)--(0.91015625,3.3959589813286076e-2)--(0.9140625,3.2809558543087175e-2)--(0.91796875,3.166100769688199e-2)--(0.921875,3.0511099586834615e-2)--(0.92578125,2.935690017471202e-2)--(0.9296875,2.8195374332281965e-2)--(0.93359375,2.702338183912779e-2)--(0.9375,2.5837674370953752e-2)--(0.94140625,2.4634893758889206e-2)--(0.9453125,2.3411571826550747e-2)--(0.94921875,2.2164132134922795e-2)--(0.953125,2.0888893983663656e-2)--(0.95703125,1.958207902838213e-2)--(0.9609375,1.823982087458487e-2)--(0.96484375,1.6858177996562345e-2)--(0.96875,1.5433150300838564e-2)--(0.97265625,1.396069960535211e-2)--(0.9765625,1.2436774234372845e-2)--(0.98046875,1.0857337833087627e-2)--(0.984375,9.218402383523575e-3)--(0.98828125,7.516065254672036e-3)--(0.9921875,5.746549947122134e-3)--(0.99609375,3.9062499999629532e-3)}
\newcommand{\serptAbbaA}{(0.0,0.1629718048254693)--(3.90625e-3,0.1627859056620267)--(7.8125e-3,0.16339450299943234)--(1.171875e-2,0.16492029668200395)--(1.5625e-2,0.16750165328727043)--(1.953125e-2,0.17129583162753584)--(2.34375e-2,0.17648263197551164)--(2.734375e-2,0.18326812299861442)--(3.125e-2,0.1918878424311025)--(3.515625e-2,0.2026084879695593)--(3.90625e-2,0.2157265780982795)--(4.296875e-2,0.23156185978527227)--(4.6875e-2,0.2504424397916655)--(5.078125e-2,0.2726779511529478)--(5.46875e-2,0.2985170498907936)--(5.859375e-2,0.328087054938826)--(6.25e-2,0.36131775617798617)--(6.640625e-2,0.39785918130316483)--(7.03125e-2,0.43701370289909147)--(7.421875e-2,0.47771230547373594)--(7.8125e-2,0.5185655092002511)--(8.203125e-2,0.5580035954336073)--(8.59375e-2,0.5944882440983787)--(8.984375e-2,0.6267421698247079)--(9.375e-2,0.6539273343516825)--(9.765625e-2,0.6757197511113748)--(0.1015625,0.6922710189864296)--(0.10546875,0.7040879810685231)--(0.109375,0.711880943444911)--(0.11328125,0.7164247485193191)--(0.1171875,0.7184573490762239)--(0.12109375,0.7186209850181191)--(0.125,0.7174388561881925)--(0.12890625,0.715315808337001)--(0.1328125,0.7125522499277158)--(0.13671875,0.7093633317895375)--(0.140625,0.7058984403399419)--(0.14453125,0.7022584423817403)--(0.1484375,0.6985097083669966)--(0.15234375,0.6946948596369046)--(0.15625,0.6908406353048547)--(0.16015625,0.6869634353699656)--(0.1640625,0.6830730985331964)--(0.16796875,0.6791754002906057)--(0.171875,0.6752736589680308)--(0.17578125,0.6713697410347484)--(0.1796875,0.6674646744371436)--(0.18359375,0.6635590135851517)--(0.1875,0.6596530513364187)--(0.19140625,0.6557469392195198)--(0.1953125,0.6518407540390344)--(0.19921875,0.6479345339342248)--(0.203125,0.644028297461102)--(0.20703125,0.640122053465843)--(0.2109375,0.6362158060809611)--(0.21484375,0.632309557198309)--(0.21875,0.6284033076666751)--(0.22265625,0.6244970578592863)--(0.2265625,0.620590807936997)--(0.23046875,0.6166845579677559)--(0.234375,0.6127783079797006)--(0.23828125,0.608872057984251)--(0.2421875,0.6049658079859519)--(0.24609375,0.6010595579865758)--(0.25,0.5971533079868006)--(0.25390625,0.5932470579868795)--(0.2578125,0.5893408079869072)--(0.26171875,0.5854345579869166)--(0.265625,0.5815283079869197)--(0.26953125,0.5776220579869208)--(0.2734375,0.5737158079869215)--(0.27734375,0.5698095579869213)--(0.28125,0.5659033079869213)--(0.28515625,0.5619970579869212)--(0.2890625,0.5580908079869212)--(0.29296875,0.5541845579869217)--(0.296875,0.5502783079869223)--(0.30078125,0.5463720579869236)--(0.3046875,0.5424658079869253)--(0.30859375,0.5385595579869277)--(0.3125,0.5346533079869311)--(0.31640625,0.5307470579869362)--(0.3203125,0.5268408079869441)--(0.32421875,0.5229345579869558)--(0.328125,0.5190283079869729)--(0.33203125,0.5151220579869987)--(0.3359375,0.5112158079870369)--(0.33984375,0.5073095579870938)--(0.34375,0.5034033079871774)--(0.34765625,0.4994970579873003)--(0.3515625,0.49559080798748045)--(0.35546875,0.491684557987744)--(0.359375,0.48777830798812827)--(0.36328125,0.4838720579886862)--(0.3671875,0.47996580798949445)--(0.37109375,0.476059557990662)--(0.375,0.4721533079923423)--(0.37890625,0.4682470579947537)--(0.3828125,0.46434080799820415)--(0.38671875,0.4604345580031248)--(0.390625,0.4565283080101208)--(0.39453125,0.45262205802003674)--(0.3984375,0.44871580803404654)--(0.40234375,0.44480955805377936)--(0.40625,0.4409033080814858)--(0.41015625,0.43699705812026624)--(0.4140625,0.43309080817437756)--(0.41796875,0.42918455824964374)--(0.421875,0.4252783083540077)--(0.42578125,0.42137205849826587)--(0.4296875,0.4174658086970432)--(0.43359375,0.413559558970086)--(0.4375,0.40965330934396404)--(0.44140625,0.4057470598543098)--(0.4453125,0.40184081054874726)--(0.44921875,0.39793456149071416)--(0.453125,0.39402831276442496)--(0.45703125,0.390122064481297)--(0.4609375,0.38621581678823624)--(0.46484375,0.38230956987827985)--(0.46875,0.3784033240042147)--(0.47265625,0.3744970794959359)--(0.4765625,0.37059083678248633)--(0.48046875,0.3666845964199302)--(0.484375,0.3627783591264641)--(0.48828125,0.3588721258264701)--(0.4921875,0.3549658977055652)--(0.49609375,0.3510596762791113)--(0.5,0.3471534634771301)--(0.50390625,0.3432472617491144)--(0.5078125,0.33934107419285575)--(0.51171875,0.3354349047121226)--(0.515625,0.33152875820882255)--(0.51953125,0.32762264081617615)--(0.5234375,0.32371656018041034)--(0.52734375,0.3198105257995522)--(0.53125,0.31590454942905327)--(0.53515625,0.3119986455651942)--(0.5390625,0.3080928320184898)--(0.54296875,0.30418713059061386)--(0.546875,0.30028156786964855)--(0.55078125,0.2963761761597096)--(0.5546875,0.2924709945621433)--(0.55859375,0.2885660702264797)--(0.5625,0.2846614597900798)--(0.56640625,0.2807572310258671)--(0.5703125,0.2768534647175778)--(0.57421875,0.2729502567815066)--(0.578125,0.2690477206526665)--(0.58203125,0.26514598995149924)--(0.5859375,0.2612452214446702)--(0.58984375,0.25734559830993736)--(0.59375,0.25344733371052075)--(0.59765625,0.2495506746787216)--(0.6015625,0.24565590630169723)--(0.60546875,0.24176335619427367)--(0.609375,0.23787339923447884)--(0.61328125,0.23398646252717756)--(0.6171875,0.230103030549904)--(0.62109375,0.22622365042290557)--(0.625,0.2223489372327961)--(0.62890625,0.21847957932637488)--(0.6328125,0.2146163434785218)--(0.63671875,0.21076007982607442)--(0.640625,0.20691172644875855)--(0.64453125,0.20307231346914528)--(0.6484375,0.1992429665368285)--(0.65234375,0.19542490955815228)--(0.65625,0.19161946653240855)--(0.66015625,0.18782806235899333)--(0.6640625,0.18405222248792358)--(0.66796875,0.18029357129866325)--(0.671875,0.1765538291094796)--(0.67578125,0.17283480774146398)--(0.6796875,0.16913840458760276)--(0.68359375,0.16546659516735546)--(0.6875,0.16182142418034928)--(0.69140625,0.15820499510808753)--(0.6953125,0.15461945844888123)--(0.69921875,0.15106699870730447)--(0.703125,0.1475498202940174)--(0.70703125,0.14407013252347103)--(0.7109375,0.1406301339245271)--(0.71484375,0.1372319961012385)--(0.71875,0.1338778473969921)--(0.72265625,0.13056975662418963)--(0.7265625,0.1273097171232222)--(0.73046875,0.12409963140855249)--(0.734375,0.12094129664647613)--(0.73828125,0.1178363911891112)--(0.7421875,0.11478646236313472)--(0.74609375,0.11179291568080862)--(0.75,0.10885700560608279)--(0.75390625,0.10597982797136207)--(0.7578125,0.10316231410220793)--(0.76171875,0.10040522666913439)--(0.765625,9.770915724898452e-2)--(0.76953125,9.507452554420329e-2)--(0.7734375,9.250158017758474e-2)--(0.77734375,8.999040095342326e-2)--(0.78125,8.75409024539543e-2)--(0.78515625,8.51528388227478e-2)--(0.7890625,8.282580957439767e-2)--(0.79296875,8.055926626227113e-2)--(0.796875,7.835251983297169e-2)--(0.80078125,7.620474849709781e-2)--(0.8046875,7.411500595034463e-2)--(0.80859375,7.208222978644536e-2)--(0.8125,7.010524995327376e-2)--(0.81640625,6.818279711507466e-2)--(0.8203125,6.631351079666706e-2)--(0.82421875,6.449594719908866e-2)--(0.828125,6.272858659004715e-2)--(0.83203125,6.100984018633077e-2)--(0.8359375,5.933805645869527e-2)--(0.83984375,5.771152680243081e-2)--(0.84375,5.612849052865861e-2)--(0.84765625,5.458713914229344e-2)--(0.8515625,5.308561988250209e-2)--(0.85546875,5.1622038510381545e-2)--(0.859375,5.019446133655475e-2)--(0.86328125,4.880091648851409e-2)--(0.8671875,4.7439394423992996e-2)--(0.87109375,4.6107847702572466e-2)--(0.875,4.48041900333272e-2)--(0.87890625,4.352629462182325e-2)--(0.8828125,4.227199184540707e-2)--(0.88671875,4.10390662917622e-2)--(0.890625,3.982525320237899e-2)--(0.89453125,3.8628234370218444e-2)--(0.8984375,3.744563354965458e-2)--(0.90234375,3.627501144709701e-2)--(0.90625,3.5113860372722926e-2)--(0.91015625,3.395959864776806e-2)--(0.9140625,3.2809564877980923e-2)--(0.91796875,3.1661012222313004e-2)--(0.921875,3.0511102806696406e-2)--(0.92578125,2.9356902455807136e-2)--(0.9296875,2.8195375940788924e-2)--(0.93359375,2.7023382967584247e-2)--(0.9375,2.5837675158170294e-2)--(0.94140625,2.463489430459574e-2)--(0.9453125,2.341157220213419e-2)--(0.94921875,2.2164132391298785e-2)--(0.953125,2.088889415698498e-2)--(0.95703125,1.958207914421507e-2)--(0.9609375,1.8239820950924666e-2)--(0.96484375,1.6858178046009895e-2)--(0.96875,1.5433150332173025e-2)--(0.97265625,1.3960699624651475e-2)--(0.9765625,1.2436774245793352e-2)--(0.98046875,1.085733783948005e-2)--(0.984375,9.218402386799513e-3)--(0.98828125,7.516065256109588e-3)--(0.9921875,5.746549947598365e-3)--(0.99609375,3.9062499999958883e-3)}
\newcommand{\serptAbbaB}{(0.0,0.32928571478198054)--(3.90625e-3,0.3253794652461034)--(7.8125e-3,0.3214732160250095)--(1.171875e-2,0.3175669673209693)--(1.5625e-2,0.313660719458689)--(1.953125e-2,0.3097544729546052)--(2.34375e-2,0.3058482286224854)--(2.734375e-2,0.30194198773268527)--(3.125e-2,0.29803575224982015)--(3.515625e-2,0.29412952518371227)--(3.90625e-2,0.29022331110207134)--(4.296875e-2,0.28631711687134875)--(4.6875e-2,0.2824109527156011)--(5.078125e-2,0.2785048337130665)--(5.46875e-2,0.27459878188755377)--(5.859375e-2,0.2706928290975541)--(6.25e-2,0.2667870209807625)--(6.640625e-2,0.2628814222754163)--(7.03125e-2,0.25897612391162284)--(7.421875e-2,0.2550712523435326)--(7.8125e-2,0.25116698167311075)--(8.203125e-2,0.24726354919271532)--(8.59375e-2,0.2433612750388246)--(8.984375e-2,0.23946058669284645)--(9.375e-2,0.2355620490745306)--(9.765625e-2,0.23166640093488813)--(0.1015625,0.22777459815368223)--(0.10546875,0.22388786436713431)--(0.109375,0.22000774908283935)--(0.11328125,0.21613619307459053)--(0.1171875,0.21227560039159407)--(0.12109375,0.20842891577710143)--(0.125,0.20459970569686367)--(0.12890625,0.20079224056876518)--(0.1328125,0.19701157521645046)--(0.13671875,0.19326362410806266)--(0.140625,0.18955522765851984)--(0.14453125,0.18589420583985478)--(0.1484375,0.18228939561611726)--(0.15234375,0.17875066933047454)--(0.15625,0.17528893212183266)--(0.16015625,0.17191609769502705)--(0.1640625,0.16864504322812104)--(0.16796875,0.1654895457500744)--(0.171875,0.1624642038123695)--(0.17578125,0.15958434954888115)--(0.1796875,0.15686595711783213)--(0.18359375,0.1543255539239505)--(0.1875,0.15198014084551015)--(0.19140625,0.14984712690627805)--(0.1953125,0.14794428245038777)--(0.19921875,0.14628971295035265)--(0.203125,0.14490185317812676)--(0.20703125,0.14379947867285958)--(0.2109375,0.14300172830947266)--(0.21484375,0.1425281283467357)--(0.21875,0.14239860462175066)--(0.22265625,0.14263346555140669)--(0.2265625,0.14325333429911782)--(0.23046875,0.1442790039147155)--(0.234375,0.14573118461551304)--(0.23828125,0.14763010800055917)--(0.2421875,0.14999494952965095)--(0.24609375,0.15284302912081524)--(0.25,0.15618875181689829)--(0.25390625,0.16004225832271585)--(0.2578125,0.1644077715276816)--(0.26171875,0.1692816528620449)--(0.265625,0.17465022405771932)--(0.26953125,0.18048746667304635)--(0.2734375,0.18675278157764147)--(0.27734375,0.19338906648464121)--(0.28125,0.20032143800952698)--(0.28515625,0.2074569652730692)--(0.2890625,0.21468577002568787)--(0.29296875,0.22188376069520307)--(0.296875,0.2289170930740717)--(0.30078125,0.23564819894248443)--(0.3046875,0.24194293469969946)--(0.30859375,0.24767813945762762)--(0.3125,0.25274873015401794)--(0.31640625,0.257073458586083)--(0.3203125,0.2605986299305273)--(0.32421875,0.2632994001479604)--(0.328125,0.2651786532113059)--(0.33203125,0.26626381444584307)--(0.3359375,0.266602205440187)--(0.33984375,0.26625565006793145)--(0.34375,0.265295005626323)--(0.34765625,0.26379515656087915)--(0.3515625,0.2618308229942671)--(0.35546875,0.2594733502050516)--(0.359375,0.2567884910072563)--(0.36328125,0.2538350856367219)--(0.3671875,0.2506644837701259)--(0.37109375,0.24732053240220014)--(0.375,0.24383995977221162)--(0.37890625,0.24025300798336283)--(0.3828125,0.23658419631229177)--(0.38671875,0.23285312722564475)--(0.390625,0.2290752741539094)--(0.39453125,0.22526271242926846)--(0.3984375,0.22142477208640476)--(0.40234375,0.21756860381647614)--(0.40625,0.21369965797353258)--(0.41015625,0.2098220819806788)--(0.4140625,0.20593904455184747)--(0.41796875,0.20205299650875)--(0.421875,0.19816587817764172)--(0.42578125,0.19427928281838372)--(0.4296875,0.19039458458083142)--(0.43359375,0.18651303832256796)--(0.4375,0.1826358574081501)--(0.44140625,0.1787642744401637)--(0.4453125,0.17489958880385698)--(0.44921875,0.1710432039694432)--(0.453125,0.1671966567001608)--(0.45703125,0.1633616396587777)--(0.4609375,0.15954001838250675)--(0.46484375,0.15573384319488653)--(0.46875,0.15194535633044998)--(0.47265625,0.14817699435130505)--(0.4765625,0.14443138582195747)--(0.48046875,0.1407113441682564)--(0.484375,0.1370198556670583)--(0.48828125,0.13336006258396296)--(0.4921875,0.12973524158591143)--(0.49609375,0.12614877769185695)--(0.5,0.1226041341760101)--(0.50390625,0.119104818992172)--(0.5078125,0.11565434843249814)--(0.51171875,0.1122562088587126)--(0.515625,0.1089138174388087)--(0.51953125,0.10563048288029163)--(0.5234375,0.10240936716729365)--(0.52734375,9.92534492816416e-2)--(0.53125,9.61654918184406e-2)--(0.53515625,9.31480112990568e-2)--(0.5390625,9.02032528451251e-2)--(0.54296875,8.733316971476002e-2)--(0.546875,8.453940802603967e-2)--(0.55078125,8.182329681287087e-2)--(0.5546875,7.918584338389927e-2)--(0.55859375,7.662773379448447e-2)--(0.5625,7.414933810158106e-2)--(0.56640625,7.175071995644729e-2)--(0.5703125,6.943165000322074e-2)--(0.57421875,6.719162249337982e-2)--(0.578125,6.502987449607996e-2)--(0.58203125,6.294540707998958e-2)--(0.5859375,6.09370078602195e-2)--(0.58984375,5.900327434023578e-2)--(0.59375,5.7142637528958914e-2)--(0.59765625,5.53533853733124e-2)--(0.6015625,5.3633685612281906e-2)--(0.60546875,5.1981607726515e-2)--(0.609375,5.039514372465155e-2)--(0.61328125,4.887222757153793e-2)--(0.6171875,4.741075312247893e-2)--(0.62109375,4.600859048054032e-2)--(0.625,4.466360073993321e-2)--(0.62890625,4.337364911745672e-2)--(0.6328125,4.2136616505924616e-2)--(0.63671875,4.095040950881197e-2)--(0.640625,3.981296903457644e-2)--(0.64453125,3.8722277542852346e-2)--(0.6484375,3.7676365043721675e-2)--(0.65234375,3.667331395624054e-2)--(0.65625,3.571126293403421e-2)--(0.66015625,3.478840976472889e-2)--(0.6640625,3.390301344686743e-2)--(0.66796875,3.3053395543242686e-2)--(0.671875,3.2237940903809825e-2)--(0.67578125,3.145509784477954e-2)--(0.6796875,3.070337786356875e-2)--(0.68359375,2.9981354962183942e-2)--(0.6875,2.928766464453944e-2)--(0.69140625,2.862100264637924e-2)--(0.6953125,2.7980123449874595e-2)--(0.69921875,2.7363838628798355e-2)--(0.703125,2.67710150644667e-2)--(0.70703125,2.6200573067267554e-2)--(0.7109375,2.5651484433860318e-2)--(0.71484375,2.5122770465673648e-2)--(0.71875,2.4613499970517216e-2)--(0.72265625,2.4122787265491257e-2)--(0.7265625,2.3649790196486692e-2)--(0.73046875,2.319370818658566e-2)--(0.734375,2.2753780323601397e-2)--(0.73828125,2.232928349461854e-2)--(0.7421875,2.1919530573926836e-2)--(0.74609375,2.1523868668877566e-2)--(0.75,2.1141677427146188e-2)--(0.75390625,2.0772367407721017e-2)--(0.7578125,2.0415378516803005e-2)--(0.76171875,2.007017850933571e-2)--(0.765625,1.9736261555994013e-2)--(0.76953125,1.9413146875165783e-2)--(0.7734375,1.9100377428446422e-2)--(0.77734375,1.8797518678803533e-2)--(0.78125,1.850415740969063e-2)--(0.78515625,1.8219900602337392e-2)--(0.7890625,1.794437437096785e-2)--(0.79296875,1.7677222951883807e-2)--(0.796875,1.7418107744923823e-2)--(0.80078125,1.7166706406148334e-2)--(0.8046875,1.692271198803543e-2)--(0.80859375,1.6685832123740373e-2)--(0.8125,1.645578825633102e-2)--(0.81640625,1.6232314909775267e-2)--(0.8203125,1.6015158993885285e-2)--(0.82421875,1.580407915061361e-2)--(0.828125,1.5598845129465341e-2)--(0.83203125,1.5399237198410546e-2)--(0.8359375,1.5205045571744399e-2)--(0.83984375,1.5016069876442401e-2)--(0.84375,1.4832118625167404e-2)--(0.84765625,1.4653008717188484e-2)--(0.8515625,1.4478564920629938e-2)--(0.85546875,1.4308619403901405e-2)--(0.859375,1.4143011225809961e-2)--(0.86328125,1.3981585737724317e-2)--(0.8671875,1.3824194132439047e-2)--(0.87109375,1.3670692667898944e-2)--(0.875,1.3520941985139076e-2)--(0.87890625,1.3374806149716882e-2)--(0.8828125,1.32321513976885e-2)--(0.88671875,1.30928449115985e-2)--(0.890625,1.2956752454887092e-2)--(0.89453125,1.2823735682711286e-2)--(0.8984375,1.2693649054185156e-2)--(0.90234375,1.2566333433557609e-2)--(0.90625,1.2441608563353372e-2)--(0.91015625,1.2319265899896731e-2)--(0.9140625,1.2199050172700383e-2)--(0.91796875,1.2080639720640569e-2)--(0.921875,1.1963622519491011e-2)--(0.92578125,1.1847442672638396e-2)--(0.9296875,1.17313615454871e-2)--(0.93359375,1.1614376894470325e-2)--(0.9375,1.149507093046817e-2)--(0.94140625,1.1371567755219551e-2)--(0.9453125,1.1241184048512699e-2)--(0.94921875,1.1100228901084957e-2)--(0.953125,1.094376726049613e-2)--(0.95703125,1.076476860384623e-2)--(0.9609375,1.0554030563348221e-2)--(0.96484375,1.0299830800186245e-2)--(0.96875,9.985834621095051e-3)--(0.97265625,9.592401372007696e-3)--(0.9765625,9.093378987952861e-3)--(0.98046875,8.460149284308225e-3)--(0.984375,7.6616406753254535e-3)--(0.98828125,6.658631818000718e-3)--(0.9921875,5.421143439730217e-3)--(0.99609375,3.904665314401623e-3)}
\newcommand{\gittinsAbbaA}{(0.0,6.22298143193587e-2)--(3.90625e-3,5.907697911745354e-2)--(7.8125e-3,5.6132101413789305e-2)--(1.171875e-2,5.3401048632439545e-2)--(1.5625e-2,5.091822978566244e-2)--(1.953125e-2,4.8644031367886816e-2)--(2.34375e-2,4.6607690257661184e-2)--(2.734375e-2,4.480895386599281e-2)--(3.125e-2,4.321315511208195e-2)--(3.515625e-2,4.187004810532915e-2)--(3.90625e-2,4.07020443699329e-2)--(4.296875e-2,3.977996900339757e-2)--(4.6875e-2,3.903121149916771e-2)--(5.078125e-2,3.850952386456939e-2)--(5.46875e-2,3.815135624664447e-2)--(5.859375e-2,3.800520608115966e-2)--(6.25e-2,3.8423405601328e-2)--(6.640625e-2,3.96436179306888e-2)--(7.03125e-2,4.1835441337553826e-2)--(7.421875e-2,4.525628334720945e-2)--(7.8125e-2,5.028803608682578e-2)--(8.203125e-2,5.749363793023769e-2)--(8.59375e-2,6.77046378149971e-2)--(8.984375e-2,8.215784610234057e-2)--(9.375e-2,0.10271078661243403)--(9.765625e-2,0.13218532592427196)--(0.1015625,0.17492250703538983)--(0.10546875,0.2376899269684202)--(0.109375,0.33118531764120773)--(0.11328125,0.47256181864453656)--(0.1171875,0.6897277375345434)--(0.12109375,0.7186209850181191)--(0.125,0.7174388561881925)--(0.12890625,0.715315808337001)--(0.1328125,0.7125522499277158)--(0.13671875,0.7093633317895375)--(0.140625,0.7058984403399419)--(0.14453125,0.7022584423817403)--(0.1484375,0.6985097083669966)--(0.15234375,0.6946948596369046)--(0.15625,0.6908406353048547)--(0.16015625,0.6869634353699656)--(0.1640625,0.6830730985331964)--(0.16796875,0.6791754002906057)--(0.171875,0.6752736589680308)--(0.17578125,0.6713697410347484)--(0.1796875,0.6674646744371436)--(0.18359375,0.6635590135851517)--(0.1875,0.6596530513364187)--(0.19140625,0.6557469392195198)--(0.1953125,0.6518407540390344)--(0.19921875,0.6479345339342248)--(0.203125,0.644028297461102)--(0.20703125,0.640122053465843)--(0.2109375,0.6362158060809611)--(0.21484375,0.632309557198309)--(0.21875,0.6284033076666751)--(0.22265625,0.6244970578592863)--(0.2265625,0.620590807936997)--(0.23046875,0.6166845579677559)--(0.234375,0.6127783079797006)--(0.23828125,0.608872057984251)--(0.2421875,0.6049658079859519)--(0.24609375,0.6010595579865758)--(0.25,0.5971533079868006)--(0.25390625,0.5932470579868795)--(0.2578125,0.5893408079869072)--(0.26171875,0.5854345579869166)--(0.265625,0.5815283079869197)--(0.26953125,0.5776220579869208)--(0.2734375,0.5737158079869215)--(0.27734375,0.5698095579869213)--(0.28125,0.5659033079869213)--(0.28515625,0.5619970579869212)--(0.2890625,0.5580908079869212)--(0.29296875,0.5541845579869217)--(0.296875,0.5502783079869223)--(0.30078125,0.5463720579869236)--(0.3046875,0.5424658079869253)--(0.30859375,0.5385595579869277)--(0.3125,0.5346533079869311)--(0.31640625,0.5307470579869362)--(0.3203125,0.5268408079869441)--(0.32421875,0.5229345579869558)--(0.328125,0.5190283079869729)--(0.33203125,0.5151220579869987)--(0.3359375,0.5112158079870369)--(0.33984375,0.5073095579870938)--(0.34375,0.5034033079871774)--(0.34765625,0.4994970579873003)--(0.3515625,0.49559080798748045)--(0.35546875,0.491684557987744)--(0.359375,0.48777830798812827)--(0.36328125,0.4838720579886862)--(0.3671875,0.47996580798949445)--(0.37109375,0.476059557990662)--(0.375,0.4721533079923423)--(0.37890625,0.4682470579947537)--(0.3828125,0.46434080799820415)--(0.38671875,0.4604345580031248)--(0.390625,0.4565283080101208)--(0.39453125,0.45262205802003674)--(0.3984375,0.44871580803404654)--(0.40234375,0.44480955805377936)--(0.40625,0.4409033080814858)--(0.41015625,0.43699705812026624)--(0.4140625,0.43309080817437756)--(0.41796875,0.42918455824964374)--(0.421875,0.4252783083540077)--(0.42578125,0.42137205849826587)--(0.4296875,0.4174658086970432)--(0.43359375,0.413559558970086)--(0.4375,0.40965330934396404)--(0.44140625,0.4057470598543098)--(0.4453125,0.40184081054874726)--(0.44921875,0.39793456149071416)--(0.453125,0.39402831276442496)--(0.45703125,0.390122064481297)--(0.4609375,0.38621581678823624)--(0.46484375,0.38230956987827985)--(0.46875,0.3784033240042147)--(0.47265625,0.3744970794959359)--(0.4765625,0.37059083678248633)--(0.48046875,0.3666845964199302)--(0.484375,0.3627783591264641)--(0.48828125,0.3588721258264701)--(0.4921875,0.3549658977055652)--(0.49609375,0.3510596762791113)--(0.5,0.3471534634771301)--(0.50390625,0.3432472617491144)--(0.5078125,0.33934107419285575)--(0.51171875,0.3354349047121226)--(0.515625,0.33152875820882255)--(0.51953125,0.32762264081617615)--(0.5234375,0.32371656018041034)--(0.52734375,0.3198105257995522)--(0.53125,0.31590454942905327)--(0.53515625,0.3119986455651942)--(0.5390625,0.3080928320184898)--(0.54296875,0.30418713059061386)--(0.546875,0.30028156786964855)--(0.55078125,0.2963761761597096)--(0.5546875,0.2924709945621433)--(0.55859375,0.2885660702264797)--(0.5625,0.2846614597900798)--(0.56640625,0.2807572310258671)--(0.5703125,0.2768534647175778)--(0.57421875,0.2729502567815066)--(0.578125,0.2690477206526665)--(0.58203125,0.26514598995149924)--(0.5859375,0.2612452214446702)--(0.58984375,0.25734559830993736)--(0.59375,0.25344733371052075)--(0.59765625,0.2495506746787216)--(0.6015625,0.24565590630169723)--(0.60546875,0.24176335619427367)--(0.609375,0.23787339923447884)--(0.61328125,0.23398646252717756)--(0.6171875,0.230103030549904)--(0.62109375,0.22622365042290557)--(0.625,0.2223489372327961)--(0.62890625,0.21847957932637488)--(0.6328125,0.2146163434785218)--(0.63671875,0.21076007982607442)--(0.640625,0.20691172644875855)--(0.64453125,0.20307231346914528)--(0.6484375,0.1992429665368285)--(0.65234375,0.19542490955815228)--(0.65625,0.19161946653240855)--(0.66015625,0.18782806235899333)--(0.6640625,0.18405222248792358)--(0.66796875,0.18029357129866325)--(0.671875,0.1765538291094796)--(0.67578125,0.17283480774146398)--(0.6796875,0.16913840458760276)--(0.68359375,0.16546659516735546)--(0.6875,0.16182142418034928)--(0.69140625,0.15820499510808753)--(0.6953125,0.15461945844888123)--(0.69921875,0.15106699870730447)--(0.703125,0.1475498202940174)--(0.70703125,0.14407013252347103)--(0.7109375,0.1406301339245271)--(0.71484375,0.1372319961012385)--(0.71875,0.1338778473969921)--(0.72265625,0.13056975662418963)--(0.7265625,0.1273097171232222)--(0.73046875,0.12409963140855249)--(0.734375,0.12094129664647613)--(0.73828125,0.1178363911891112)--(0.7421875,0.11478646236313472)--(0.74609375,0.11179291568080862)--(0.75,0.10885700560608279)--(0.75390625,0.10597982797136207)--(0.7578125,0.10316231410220793)--(0.76171875,0.10040522666913439)--(0.765625,9.770915724898452e-2)--(0.76953125,9.507452554420329e-2)--(0.7734375,9.250158017758474e-2)--(0.77734375,8.999040095342326e-2)--(0.78125,8.75409024539543e-2)--(0.78515625,8.51528388227478e-2)--(0.7890625,8.282580957439767e-2)--(0.79296875,8.055926626227113e-2)--(0.796875,7.835251983297169e-2)--(0.80078125,7.620474849709781e-2)--(0.8046875,7.411500595034463e-2)--(0.80859375,7.208222978644536e-2)--(0.8125,7.010524995327376e-2)--(0.81640625,6.818279711507466e-2)--(0.8203125,6.631351079666706e-2)--(0.82421875,6.449594719908866e-2)--(0.828125,6.272858659004715e-2)--(0.83203125,6.100984018633077e-2)--(0.8359375,5.933805645869527e-2)--(0.83984375,5.771152680243081e-2)--(0.84375,5.612849052865861e-2)--(0.84765625,5.458713914229344e-2)--(0.8515625,5.308561988250209e-2)--(0.85546875,5.1622038510381545e-2)--(0.859375,5.019446133655475e-2)--(0.86328125,4.880091648851409e-2)--(0.8671875,4.7439394423992996e-2)--(0.87109375,4.6107847702572466e-2)--(0.875,4.48041900333272e-2)--(0.87890625,4.352629462182325e-2)--(0.8828125,4.227199184540707e-2)--(0.88671875,4.10390662917622e-2)--(0.890625,3.982525320237899e-2)--(0.89453125,3.8628234370218444e-2)--(0.8984375,3.744563354965458e-2)--(0.90234375,3.627501144709701e-2)--(0.90625,3.5113860372722926e-2)--(0.91015625,3.395959864776806e-2)--(0.9140625,3.2809564877980923e-2)--(0.91796875,3.1661012222313004e-2)--(0.921875,3.0511102806696406e-2)--(0.92578125,2.9356902455807136e-2)--(0.9296875,2.8195375940788924e-2)--(0.93359375,2.7023382967584247e-2)--(0.9375,2.5837675158170294e-2)--(0.94140625,2.463489430459574e-2)--(0.9453125,2.341157220213419e-2)--(0.94921875,2.2164132391298785e-2)--(0.953125,2.088889415698498e-2)--(0.95703125,1.958207914421507e-2)--(0.9609375,1.8239820950924666e-2)--(0.96484375,1.6858178046009895e-2)--(0.96875,1.5433150332173025e-2)--(0.97265625,1.3960699624651475e-2)--(0.9765625,1.2436774245793352e-2)--(0.98046875,1.085733783948005e-2)--(0.984375,9.218402386799513e-3)--(0.98828125,7.516065256109588e-3)--(0.9921875,5.746549947598365e-3)--(0.99609375,3.9062499999958883e-3)}
\newcommand{\gittinsAbbaB}{(0.0,0.32928571478198054)--(3.90625e-3,0.3253794652461034)--(7.8125e-3,0.3214732160250095)--(1.171875e-2,0.3175669673209693)--(1.5625e-2,0.313660719458689)--(1.953125e-2,0.3097544729546052)--(2.34375e-2,0.3058482286224854)--(2.734375e-2,0.30194198773268527)--(3.125e-2,0.29803575224982015)--(3.515625e-2,0.29412952518371227)--(3.90625e-2,0.29022331110207134)--(4.296875e-2,0.28631711687134875)--(4.6875e-2,0.2824109527156011)--(5.078125e-2,0.2785048337130665)--(5.46875e-2,0.27459878188755377)--(5.859375e-2,0.2706928290975541)--(6.25e-2,0.2667870209807625)--(6.640625e-2,0.2617743587263647)--(7.03125e-2,0.25670708624878313)--(7.421875e-2,0.2516403487750621)--(7.8125e-2,0.2465743599390019)--(8.203125e-2,0.24149083974189484)--(8.59375e-2,0.2364028183984479)--(8.984375e-2,0.23131674102820016)--(9.375e-2,0.2262332803567325)--(9.765625e-2,0.22115330749242523)--(0.1015625,0.2160779378118791)--(0.10546875,0.2110085832268672)--(0.109375,0.2059328190889752)--(0.11328125,0.20085169604264957)--(0.1171875,0.19578326424634362)--(0.12109375,0.19073075497139777)--(0.125,0.1856980179296042)--(0.12890625,0.18068958142729574)--(0.1328125,0.17568731508481797)--(0.13671875,0.17070926145978918)--(0.140625,0.1657737944321762)--(0.14453125,0.16088852094155812)--(0.1484375,0.15606179798234948)--(0.15234375,0.15126587757268778)--(0.15625,0.1465443077608148)--(0.16015625,0.14191054585114163)--(0.1640625,0.1373751101324336)--(0.16796875,0.13290781559104717)--(0.171875,0.1285569259734399)--(0.17578125,0.12433700537041809)--(0.1796875,0.12023701600830977)--(0.18359375,0.11626054301677669)--(0.1875,0.11244498880636919)--(0.19140625,0.10878113305218001)--(0.1953125,0.10525887588596858)--(0.19921875,0.10192095599827049)--(0.203125,9.874405460232541e-2)--(0.20703125,9.573435465400029e-2)--(0.2109375,9.29242369860347e-2)--(0.21484375,9.02619039264915e-2)--(0.21875,8.779878233128047e-2)--(0.22265625,8.551349491419714e-2)--(0.2265625,8.340078232853373e-2)--(0.23046875,8.148817066320942e-2)--(0.234375,7.972458750844538e-2)--(0.23828125,7.817071189149978e-2)--(0.2421875,7.675758836482349e-2)--(0.24609375,7.554713367646593e-2)--(0.25,7.448246225659444e-2)--(0.25390625,7.360750038542482e-2)--(0.2578125,7.28786690630172e-2)--(0.26171875,7.232959228728912e-2)--(0.265625,7.192302051546785e-2)--(0.26953125,7.168834764965315e-2)--(0.2734375,7.165506660585613e-2)--(0.27734375,7.219604591119443e-2)--(0.28125,7.339205919989389e-2)--(0.28515625,7.531317158235014e-2)--(0.2890625,7.805427367898346e-2)--(0.29296875,8.17405421753477e-2)--(0.296875,8.653473555890784e-2)--(0.30078125,9.264688836588564e-2)--(0.3046875,0.10034717338281088)--(0.30859375,0.10998298405374837)--(0.3125,0.12200168010280528)--(0.31640625,0.1369809826389584)--(0.3203125,0.15566976458073722)--(0.32421875,0.17904304997596238)--(0.328125,0.20837654448953122)--(0.33203125,0.24534816169104673)--(0.3359375,0.266602205440187)--(0.33984375,0.26625565006793145)--(0.34375,0.265295005626323)--(0.34765625,0.26379515656087915)--(0.3515625,0.2618308229942671)--(0.35546875,0.2594733502050516)--(0.359375,0.2567884910072563)--(0.36328125,0.2538350856367219)--(0.3671875,0.2506644837701259)--(0.37109375,0.24732053240220014)--(0.375,0.24383995977221162)--(0.37890625,0.24025300798336283)--(0.3828125,0.23658419631229177)--(0.38671875,0.23285312722564475)--(0.390625,0.2290752741539094)--(0.39453125,0.22526271242926846)--(0.3984375,0.22142477208640476)--(0.40234375,0.21756860381647614)--(0.40625,0.21369965797353258)--(0.41015625,0.2098220819806788)--(0.4140625,0.20593904455184747)--(0.41796875,0.20205299650875)--(0.421875,0.19816587817764172)--(0.42578125,0.19427928281838372)--(0.4296875,0.19039458458083142)--(0.43359375,0.18651303832256796)--(0.4375,0.1826358574081501)--(0.44140625,0.1787642744401637)--(0.4453125,0.17489958880385698)--(0.44921875,0.1710432039694432)--(0.453125,0.1671966567001608)--(0.45703125,0.1633616396587777)--(0.4609375,0.15954001838250675)--(0.46484375,0.15573384319488653)--(0.46875,0.15194535633044998)--(0.47265625,0.14817699435130505)--(0.4765625,0.14443138582195747)--(0.48046875,0.1407113441682564)--(0.484375,0.1370198556670583)--(0.48828125,0.13336006258396296)--(0.4921875,0.12973524158591143)--(0.49609375,0.12614877769185695)--(0.5,0.1226041341760101)--(0.50390625,0.119104818992172)--(0.5078125,0.11565434843249814)--(0.51171875,0.1122562088587126)--(0.515625,0.1089138174388087)--(0.51953125,0.10563048288029163)--(0.5234375,0.10240936716729365)--(0.52734375,9.92534492816416e-2)--(0.53125,9.61654918184406e-2)--(0.53515625,9.31480112990568e-2)--(0.5390625,9.02032528451251e-2)--(0.54296875,8.733316971476002e-2)--(0.546875,8.453940802603967e-2)--(0.55078125,8.182329681287087e-2)--(0.5546875,7.918584338389927e-2)--(0.55859375,7.662773379448447e-2)--(0.5625,7.414933810158106e-2)--(0.56640625,7.175071995644729e-2)--(0.5703125,6.943165000322074e-2)--(0.57421875,6.719162249337982e-2)--(0.578125,6.502987449607996e-2)--(0.58203125,6.294540707998958e-2)--(0.5859375,6.09370078602195e-2)--(0.58984375,5.900327434023578e-2)--(0.59375,5.7142637528958914e-2)--(0.59765625,5.53533853733124e-2)--(0.6015625,5.3633685612281906e-2)--(0.60546875,5.1981607726515e-2)--(0.609375,5.039514372465155e-2)--(0.61328125,4.887222757153793e-2)--(0.6171875,4.741075312247893e-2)--(0.62109375,4.600859048054032e-2)--(0.625,4.466360073993321e-2)--(0.62890625,4.337364911745672e-2)--(0.6328125,4.2136616505924616e-2)--(0.63671875,4.095040950881197e-2)--(0.640625,3.981296903457644e-2)--(0.64453125,3.8722277542852346e-2)--(0.6484375,3.7676365043721675e-2)--(0.65234375,3.667331395624054e-2)--(0.65625,3.571126293403421e-2)--(0.66015625,3.478840976472889e-2)--(0.6640625,3.390301344686743e-2)--(0.66796875,3.3053395543242686e-2)--(0.671875,3.2237940903809825e-2)--(0.67578125,3.145509784477954e-2)--(0.6796875,3.070337786356875e-2)--(0.68359375,2.9981354962183942e-2)--(0.6875,2.928766464453944e-2)--(0.69140625,2.862100264637924e-2)--(0.6953125,2.7980123449874595e-2)--(0.69921875,2.7363838628798355e-2)--(0.703125,2.67710150644667e-2)--(0.70703125,2.6200573067267554e-2)--(0.7109375,2.5651484433860318e-2)--(0.71484375,2.5122770465673648e-2)--(0.71875,2.4613499970517216e-2)--(0.72265625,2.4122787265491257e-2)--(0.7265625,2.3649790196486692e-2)--(0.73046875,2.319370818658566e-2)--(0.734375,2.2753780323601397e-2)--(0.73828125,2.232928349461854e-2)--(0.7421875,2.1919530573926836e-2)--(0.74609375,2.1523868668877566e-2)--(0.75,2.1141677427146188e-2)--(0.75390625,2.0772367407721017e-2)--(0.7578125,2.0415378516803005e-2)--(0.76171875,2.007017850933571e-2)--(0.765625,1.9736261555994013e-2)--(0.76953125,1.9413146875165783e-2)--(0.7734375,1.9100377428446422e-2)--(0.77734375,1.8797518678803533e-2)--(0.78125,1.850415740969063e-2)--(0.78515625,1.8219900602337392e-2)--(0.7890625,1.794437437096785e-2)--(0.79296875,1.7677222951883807e-2)--(0.796875,1.7418107744923823e-2)--(0.80078125,1.7166706406148334e-2)--(0.8046875,1.692271198803543e-2)--(0.80859375,1.6685832123740373e-2)--(0.8125,1.645578825633102e-2)--(0.81640625,1.6232314909775267e-2)--(0.8203125,1.6015158993885285e-2)--(0.82421875,1.580407915061361e-2)--(0.828125,1.5598845129465341e-2)--(0.83203125,1.5399237198410546e-2)--(0.8359375,1.5205045571744399e-2)--(0.83984375,1.5016069876442401e-2)--(0.84375,1.4832118625167404e-2)--(0.84765625,1.4653008717188484e-2)--(0.8515625,1.4478564920629938e-2)--(0.85546875,1.4308619403901405e-2)--(0.859375,1.4143011225809961e-2)--(0.86328125,1.3981585737724317e-2)--(0.8671875,1.3824194132439047e-2)--(0.87109375,1.3670692667898944e-2)--(0.875,1.3520941985139076e-2)--(0.87890625,1.3374806149716882e-2)--(0.8828125,1.32321513976885e-2)--(0.88671875,1.30928449115985e-2)--(0.890625,1.2956752454887092e-2)--(0.89453125,1.2823735682711286e-2)--(0.8984375,1.2693649054185156e-2)--(0.90234375,1.2566333433557609e-2)--(0.90625,1.2441608563353372e-2)--(0.91015625,1.2319265899896731e-2)--(0.9140625,1.2199050172700383e-2)--(0.91796875,1.2080639720640569e-2)--(0.921875,1.1963622519491011e-2)--(0.92578125,1.1847442672638396e-2)--(0.9296875,1.17313615454871e-2)--(0.93359375,1.1614376894470325e-2)--(0.9375,1.149507093046817e-2)--(0.94140625,1.1371567755219551e-2)--(0.9453125,1.1241184048512699e-2)--(0.94921875,1.1100228901084957e-2)--(0.953125,1.094376726049613e-2)--(0.95703125,1.076476860384623e-2)--(0.9609375,1.0554030563348221e-2)--(0.96484375,1.0299830800186245e-2)--(0.96875,9.985834621095051e-3)--(0.97265625,9.592401372007696e-3)--(0.9765625,9.093378987952861e-3)--(0.98046875,8.460149284308225e-3)--(0.984375,7.6616406753254535e-3)--(0.98828125,6.658631818000718e-3)--(0.9921875,5.421143439730217e-3)--(0.99609375,3.904665314401623e-3)}


==> tikz/tikz_macros.tex <==
\makeatletter

% The calc library needs this.
\catcode`\$=3 % math shift

\usetikzlibrary{backgrounds, math, shapes, positioning,
  decorations.markings, decorations.pathreplacing, calligraphy}

\def\@above{above}
\def\@below{below}
\def\@negative{-}
\newcommand{\downmode}{%
  \def\@above{below}
  \def\@below{above}
  \def\@negative{}}

\newcommand{\xscale}{9}
\newcommand{\yscale}{9}
\newcommand{\ticksize}{2.5}
\newcommand{\arrowsize}{5}
\newcommand{\xarrowsize}{(\arrowsize/\xscale)}
\newcommand{\yarrowsize}{(\arrowsize/\yscale)}

\newcommand{\xscaleload}{%
  \renewcommand{\xscale}{150}
  \renewcommand{\yscale}{10}}

\newcommand{\projx}[1]{($ (0,0)!#1!(1,0) $)}
\newcommand{\projxheight}[2]{($ (0,#2)!#1!(1,#2) $)}
\newcommand{\midpt}[2]{($ #1!0.5!#2 $)}

\newcommand{\xguide}[3][]{%
  \draw[axis] ({#2}, 0) -- ({#2}, {\@negative(\ticksize)/\yscale})
  node[\@below] {\ifempty{#1}{$#2$}{#1}\strut};
  \draw[guide] ({#2}, 0) -- ({#2}, {#3});}
\newcommand{\yguide}[3][]{%
  \draw[axis] (0, {#3}) -- (-\ticksize/\xscale, {#3})
  node[left] {\ifempty{#1}{$#3$}{#1}};
  \draw[guide] (0, {#3}) -- ({#2}, {#3});}
\newcommand{\yguidenolabel}[2]{%
  \draw[guide] (0, {#2}) -- ({#1}, {#2});}
\newcommand{\xguidept}[2]{%
  \ifempty{#1}{}{%
    \draw[axis] \projx{#2} -- \projxheight{#2}{{\@negative(\ticksize)/\yscale}}
    node[\@below] {#1\strut}};
  \draw[guide] \projx{#2} -- #2;}

\newcommand{\axes}[6]{%
  \draw[axis, ->] (-\ticksize/\xscale, 0)
  node[left] {#3\strut} -- ({#1 + \xarrowsize}, 0) node[right] {#4\strut};
  \draw[axis, ->] (0, \@negative\ticksize/\yscale)
  node[\@below] {#5\strut} -- (0, {#2 + \yarrowsize})
  node[\@above] {#6\strut};}

\newcommand{\axesxtorsor}[4]{%
  \draw[axis, ->] (-\ticksize/\xscale, 0)
  node[left] {$0$} -- ({#1 + \xarrowsize}, 0) node[right] {#3};
  \draw[axis, ->] (0, 0) -- (0, {#2 + \yarrowsize})
  node[\@above] {#4};}

\newcommand{\point}[2][primary]{%
  \filldraw[#1, very thick] #2 circle (1.8mu);}

\newcommand{\jump}[4][primary]{%
  \point[#1, fill=white]{(#2, #3)}
  \point[#1]{(#2, #4)}}

\newcommand{\plotlegend}[1][%
  $\Delta \to 0$ limit \\ (lower bound)]{%
  \node[anchor=west, align=left] at (1.13, 32) {%
    $\Delta = 0$ \\ (exact analysis)};
  \draw[primary] (1.1, 25) -- +(0, 14);
  \node[anchor=west, align=left] at (1.13, 62) {#1};
  \draw[bubble] (1.1, 55) -- +(0, 14);}

\newcommand{\snakefirst}[2]{#1 parabola bend #1 \midpt{#1}{#2}}
\newcommand{\snakesecond}[2]{\midpt{#1}{#2} parabola bend #2 #2}
\newcommand{\snake}[2]{\snakefirst{#1}{#2} -- \snakesecond{#1}{#2}}

\newcommand{\intervallabel}[3]{%
  \begin{scope}
    \node (A) at \projx{#1} {};
    \node (B) at \projx{#2} {};
    \node[\@above=1.5pt, inner sep=0pt] at \midpt{(A)}{(B)} {%
      \footnotesize #3\vphantom{ly}};
  \end{scope}}
\newcommand{\intervalsnake}[5][--]{%
  \begin{scope}[on background layer]
    \fill[#2] \projx{#3} -- \snake{#3}{#4} -- \projx{#4};
  \end{scope}
  \draw[guide] \projx{#3} #1 \snake{#3}{#4};
  \intervallabel{#3}{#4}{#5}}
\newcommand{\intervalsnakefirst}[5][--]{%
  \begin{scope}[on background layer]
    \fill[#2] \projx{#3} -- #3 parabola bend #3 #4 -- \projx{#4};
  \end{scope}
  \draw[guide] \projx{#3} #1 #3 parabola bend #3 #4;
  \intervallabel{#3}{#4}{#5}}
\newcommand{\intervalsnakesecond}[5][--]{%
  \begin{scope}[on background layer]
    \fill[#2] \projx{#3} -- #3 parabola bend #4 #4 -- \projx{#4};
  \end{scope}
  \draw[guide] \projx{#3} #1 #3 parabola bend #4 #4;
  \intervallabel{#3}{#4}{#5}}
\newcommand{\intervalspecial}[6][--]{%
  \begin{scope}[on background layer]
    \fill[#2]
      \projx{#3}
      -- #3
      parabola bend #4 #4
      parabola bend #4 #5
      -- \projx{#5};
  \end{scope}
  \draw[guide] \projx{#3} #1 #3;
  \intervallabel{#3}{#5}{#6}}
\newcommand{\discarded}[2]{%
  \interval{discarded}{#1}{#2}{}}
\newcommand{\original}[2]{%
  \interval{original}{#1}{#2}{$0$-old}}
\newcommand{\recycled}[3][]{%
  \interval{recycled}{#2}{#3}{\ifempty{#1}{}{$#1$-}old}}

\newcommand{\Isnake}{%
  \draw[primary, name path=rank]
  \snake{(0, 3)}{(1.5, 7)}
  -- \snake{(1.5, 7)}{(2, 4)}
  -- \snake{(2, 4)}{(3.25, 12)}
  -- \snake{(3.25, 12)}{(5.25, 6)}
  -- \snake{(5.25, 6)}{(5.75, 5)}
  -- \snake{(5.75, 5)}{(8.25, 9)}
  -- \snake{(8.25, 9)}{(10.5, 3)}
  -- \snake{(10.5, 3)}{(12.5, 9)};
  \draw[primary, dotted] \snakefirst{(12.5, 9)}{(14.9, 7)};}

\tikzset{%
  figure/.style={x=\xscale, y=\yscale, thick, font=\small,
    baseline={([yshift={-\ht\strutbox}]current bounding box.north)}},
  axis/.style={semithick},
  guide/.style={black!70, opacity=0.5, densely dotted},
  primary/.style={very thick, color=purple!95!black},
  secondary/.style={very thick, color=purple!95!black},
  tertiary/.style={very thick, densely dotted, color=cyan!85!black},
  band_a/.style={fill=green!80!black!21!white},
  band_b/.style={fill=yellow!44!white},
  band_c/.style={fill=orange!90!black!28!white}}

\catcode`\$=13 % active
\makeatother

\input{tikz/hills_data}


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../soap-in-the-real-world"
%%% End:

